Whispering Pixels: Exploiting Uninitialized Register Accesses in Modern GPUs

Graphic Processing Units (GPUs) have transcended their traditional use-case of rendering graphics and nowadays also serve as a powerful platform for accelerating ubiquitous, non-graphical rendering tasks. One prominent task is inference of neural networks, which process vast amounts of personal data, such as audio, text or images. Thus, GPUs became integral components for handling vast amounts of potentially confidential data, which has awakened the interest of security researchers. This lead to the discovery of various vulnerabilities in GPUs in recent years. In this paper, we uncover yet another vulnerability class in GPUs: We found that some GPU implementations lack proper register initialization routines before shader execution, leading to unintended register content leakage of previously executed shader kernels. We showcase the existence of the aforementioned vulnerability on products of 3 major vendors - Apple, NVIDIA and Qualcomm. The vulnerability poses unique challenges to an adversary due to opaque scheduling and register remapping algorithms present in the GPU firmware, complicating the reconstruction of leaked data. In order to illustrate the real-world impact of this flaw, we showcase how these challenges can be solved for attacking various workloads on the GPU. First, we showcase how uninitialized registers leak arbitrary pixel data processed by fragment shaders. We further implement information leakage attacks on intermediate data of Convolutional Neural Networks (CNNs) and present the attack's capability to leak and reconstruct the output of Large Language Models (LLMs).

==> abstract.tex <==
\begin{abstract}
Graphic Processing Units (GPUs) have transcended their traditional use-case of rendering graphics and now serve as a powerful platform for accelerating ubiquitous, non-graphical tasks, such as training and interference of artificial intelligence. GPUs can not only be found in end-customer devices, but are they also offered as GPU-as-a-Service (GaaS) in the cloud for convenient and flexible deployment. Neural networks executed in these environments process vast amounts of potentially confidential data. Especially the recent rise of Large Language Models (LLMs) fueled the increased need for GPU hardware due to their ability of understanding and acting on natural language, a previously considered hard to solve task.\\
Consequently, vulnerabilities contained in GPUs can allow an adversary to gain tremendous insight into private user data. In this paper, we demonstrate that some GPU implementations do not properly initialize register contents prior to shader execution, leading to data leakage of previously executed shader kernels. We showcase the existence of the aforementioned vulnerability on GPUs of 3 major vendors - NVIDIA, Apple and Qualcomm. In order to indicate the real-world impact of this flaw, we first exploit this vulnerability to leak arbitrary screen pixel data. Our evaluation revealed that the presented attack is moreover capable of leaking data processed by different types of neural networks. For one, we aim to leak intermediate processed data of Convolutional Neural Networks (CNNs), which are mainly used for image classification tasks. Additionally, we present the attack's capability to leak input and output data of Large Language Models (LLMs). Our presented attack is able to leak up to TODO MB/s of stale GPU data, thus outperforming other GPU-based data leakage attacks.

\end{abstract}
